Star forming galaxies in the AKARI Deep Field South: identifications and SEDs

To investigate the nature and properties of far-infrared (FIR) sources from the AKARI Deep Field South (ADF-S), we performed an extensive search for the counterparts of 1000 ADF-S objects brighter than 0.0301 Jy in the WIDE-S (90 $\mu$m) AKARI band in the public databases (NED and SIMBAD). We analyzed the properties of the resulting sample: statistic of the identified objects, number counts, redshift distribution and morphological types. We also made a crude analysis of the clustering properties of the sources and constructed spectral energy distributions (SEDs) of 47 selected objects with the best photometry. Among 1000 investigated ADF-S sources, 545 were identified at other wavelengths. From them, 518 are known galaxies, and 343 of them were not known previously as infra-red sources. We found redshifts of 48 extragalactic objects and morphological types of 77 galaxies. We conclude that the bright FIR point sources observed in the ADF-S are mostly nearby galaxies.Their properties are very similar to properties of the local population of optically bright galaxies, except an unusually high ratio of peculiar or interacting objects and a smaller percentage of elliptical galaxies. The percentage of lenticular galaxies is the same as in the optically bright population which suggests they may frequently contain a significant amount of cool dust. It is possible that source confusion plays a significant role in more than 34% of measurements. The SEDs display a variety of galaxy types, from very actively star forming to very quiescent. Thanks to the AKARI long wavelength bands it was revealed for the first time that these galaxies form a population of objects with very cool dust.

==> points/tex_lista <==
\includegraphics[width=9cm]{points/kmalek_1.eps}
\includegraphics[width=9cm]{points/kmalek_2.eps}
\includegraphics[width=9cm]{points/kmalek_3.eps}
\includegraphics[width=9cm]{points/kmalek_4.eps}
\includegraphics[width=9cm]{points/kmalek_5.eps}
\includegraphics[width=9cm]{points/kmalek_6.eps}
\includegraphics[width=9cm]{points/kmalek_7.eps}
\includegraphics[width=9cm]{points/kmalek_8.eps}
\includegraphics[width=9cm]{points/kmalek_9.eps}
\includegraphics[width=9cm]{points/kmalek_10.eps}
\includegraphics[width=9cm]{points/kmalek_11.eps}
\includegraphics[width=9cm]{points/kmalek_12.eps}
\includegraphics[width=9cm]{points/kmalek_13.eps}
\includegraphics[width=9cm]{points/kmalek_14.eps}
\includegraphics[width=9cm]{points/kmalek_15.eps}
\includegraphics[width=9cm]{points/kmalek_16.eps}
\includegraphics[width=9cm]{points/kmalek_17.eps}
\includegraphics[width=9cm]{points/kmalek_18.eps}
\includegraphics[width=9cm]{points/kmalek_19.eps}
\includegraphics[width=9cm]{points/kmalek_20.eps}
\includegraphics[width=9cm]{points/kmalek_21.eps}
\includegraphics[width=9cm]{points/kmalek_22.eps}
\includegraphics[width=9cm]{points/kmalek_23.eps}
\includegraphics[width=9cm]{points/kmalek_24.eps}
\includegraphics[width=9cm]{points/kmalek_25.eps}
\includegraphics[width=9cm]{points/kmalek_26.eps}
\includegraphics[width=9cm]{points/kmalek_27.eps}
\includegraphics[width=9cm]{points/kmalek_28.eps}
\includegraphics[width=9cm]{points/kmalek_29.eps}
\includegraphics[width=9cm]{points/kmalek_30.eps}
\includegraphics[width=9cm]{points/kmalek_31.eps}
\includegraphics[width=9cm]{points/kmalek_32.eps}
\includegraphics[width=9cm]{points/kmalek_34.eps}
\includegraphics[width=9cm]{points/kmalek_35.eps}
\includegraphics[width=9cm]{points/kmalek_36.eps}
\includegraphics[width=9cm]{points/kmalek_37.eps}
\includegraphics[width=9cm]{points/kmalek_39.eps}
\includegraphics[width=9cm]{points/kmalek_40.eps}
\includegraphics[width=9cm]{points/kmalek_41.eps}
\includegraphics[width=9cm]{points/kmalek_42.eps}
\includegraphics[width=9cm]{points/kmalek_43.eps}
\includegraphics[width=9cm]{points/kmalek_44.ep6}
\includegraphics[width=9cm]{points/kmalek_45.eps}
\includegraphics[width=9cm]{points/kmalek_46.eps}
\includegraphics[width=9cm]{points/kmalek_47.eps}
\includegraphics[width=9cm]{points/kmalek_44.eps}
\includegraphics[width=9cm]{points/kmalek_49.eps}
\includegraphics[width=9cm]{points/kmalek_50.eps}
\includegraphics[width=9cm]{points/kmalek_51.eps}
\includegraphics[width=9cm]{points/kmalek_52.eps}
\includegraphics[width=9cm]{points/kmalek_53.eps}
\includegraphics[width=9cm]{points/kmalek_54.eps}
\includegraphics[width=9cm]{points/kmalek_55.eps}
\includegraphics[width=9cm]{points/kmalek_56.eps}
\includegraphics[width=9cm]{points/kmalek_57.eps}
\includegraphics[width=9cm]{points/kmalek_58.eps}
\includegraphics[width=9cm]{points/kmalek_59.eps}
\includegraphics[width=9cm]{points/kmalek_60.eps}
\includegraphics[width=9cm]{points/kmalek_61.eps}
\includegraphics[width=9cm]{points/kmalek_63.eps}
\includegraphics[width=9cm]{points/kmalek_64.eps}
\includegraphics[width=9cm]{points/kmalek_65.eps}
\includegraphics[width=9cm]{points/kmalek_66.eps}
\includegraphics[width=9cm]{points/kmalek_67.eps}
\includegraphics[width=9cm]{points/kmalek_68.eps}
\includegraphics[width=9cm]{points/kmalek_69.eps}
\includegraphics[width=9cm]{points/kmalek_70.eps}
\includegraphics[width=9cm]{points/kmalek_71.eps}
\includegraphics[width=9cm]{points/kmalek_72.eps}
\includegraphics[width=9cm]{points/kmalek_73.eps}
\includegraphics[width=9cm]{points/kmalek_74.eps}
\includegraphics[width=9cm]{points/kmalek_75.eps}
\includegraphics[width=9cm]{points/kmalek_76.eps}
\includegraphics[width=9cm]{points/kmalek_78.eps}
\includegraphics[width=9cm]{points/kmalek_79.eps}
\includegraphics[width=9cm]{points/kmalek_82.eps}
\includegraphics[width=9cm]{points/kmalek_83.eps}
\includegraphics[width=9cm]{points/kmalek_85.eps}
\includegraphics[width=9cm]{points/kmalek_86.eps}
\includegraphics[width=9cm]{points/kmalek_88.eps}
\includegraphics[width=9cm]{points/kmalek_89.eps}
\includegraphics[width=9cm]{points/kmalek_90.eps}
\includegraphics[width=9cm]{points/kmalek_92.eps}
\includegraphics[width=9cm]{points/kmalek_93.eps}
\includegraphics[width=9cm]{points/kmalek_94.eps}
\includegraphics[width=9cm]{points/kmalek_95.eps}
\includegraphics[width=9cm]{points/kmalek_96.eps}
\includegraphics[width=9cm]{points/kmalek_97.eps}
\includegraphics[width=9cm]{points/kmalek_98.eps}
\includegraphics[width=9cm]{points/kmalek_99.eps}
\includegraphics[width=9cm]{points/kmalek_100.eps}
\includegraphics[width=9cm]{points/kmalek_101.eps}
\includegraphics[width=9cm]{points/kmalek_102.eps}
\includegraphics[width=9cm]{points/kmalek_103.eps}
\includegraphics[width=9cm]{points/kmalek_104.eps}
\includegraphics[width=9cm]{points/kmalek_105.eps}
\includegraphics[width=9cm]{points/kmalek_106.eps}
\includegraphics[width=9cm]{points/kmalek_107.eps}
\includegraphics[width=9cm]{points/kmalek_108.eps}
\includegraphics[width=9cm]{points/kmalek_109.eps}
\includegraphics[width=9cm]{points/kmalek_110.eps}
\includegraphics[width=9cm]{points/kmalek_111.eps}
\includegraphics[width=9cm]{points/kmalek_112.eps}
\includegraphics[width=9cm]{points/kmalek_113.eps}
\includegraphics[width=9cm]{points/kmalek_114.eps}
\includegraphics[width=9cm]{points/kmalek_115.eps}
\includegraphics[width=9cm]{points/kmalek_117.eps}
\includegraphics[width=9cm]{points/kmalek_118.eps}
\includegraphics[width=9cm]{points/kmalek_119.eps}
\includegraphics[width=9cm]{points/kmalek_120.eps}
\includegraphics[width=9cm]{points/kmalek_121.eps}
\includegraphics[width=9cm]{points/kmalek_122.eps}
\includegraphics[width=9cm]{points/kmalek_123.eps}
\includegraphics[width=9cm]{points/kmalek_124.eps}
\includegraphics[width=9cm]{points/kmalek_126.eps}
\includegraphics[width=9cm]{points/kmalek_127.eps}
\includegraphics[width=9cm]{points/kmalek_130.eps}
\includegraphics[width=9cm]{points/kmalek_132.eps}
\includegraphics[width=9cm]{points/kmalek_133.eps}
\includegraphics[width=9cm]{points/kmalek_134.eps}
\includegraphics[width=9cm]{points/kmalek_135.eps}
\includegraphics[width=9cm]{points/kmalek_136.eps}
\includegraphics[width=9cm]{points/kmalek_138.eps}
\includegraphics[width=9cm]{points/kmalek_139.eps}
\includegraphics[width=9cm]{points/kmalek_140.eps}
\includegraphics[width=9cm]{points/kmalek_142.eps}
\includegraphics[width=9cm]{points/kmalek_143.eps}
\includegraphics[width=9cm]{points/kmalek_146.eps}
\includegraphics[width=9cm]{points/kmalek_147.eps}
\includegraphics[width=9cm]{points/kmalek_148.eps}
\includegraphics[width=9cm]{points/kmalek_149.eps}
\includegraphics[width=9cm]{points/kmalek_151.eps}
\includegraphics[width=9cm]{points/kmalek_152.eps}
\includegraphics[width=9cm]{points/kmalek_154.eps}
\includegraphics[width=9cm]{points/kmalek_155.eps}
\includegraphics[width=9cm]{points/kmalek_156.eps}
\includegraphics[width=9cm]{points/kmalek_158.eps}
\includegraphics[width=9cm]{points/kmalek_159.eps}
\includegraphics[width=9cm]{points/kmalek_160.eps}
\includegraphics[width=9cm]{points/kmalek_162.eps}
\includegraphics[width=9cm]{points/kmalek_165.eps}
\includegraphics[width=9cm]{points/kmalek_166.eps}
\includegraphics[width=9cm]{points/kmalek_168.eps}
\includegraphics[width=9cm]{points/kmalek_169.eps}
\includegraphics[width=9cm]{points/kmalek_170.eps}
\includegraphics[width=9cm]{points/kmalek_171.eps}
\includegraphics[width=9cm]{points/kmalek_172.eps}
\includegraphics[width=9cm]{points/kmalek_173.eps}
\includegraphics[width=9cm]{points/kmalek_175.eps}
\includegraphics[width=9cm]{points/kmalek_176.eps}
\includegraphics[width=9cm]{points/kmalek_177.eps}
\includegraphics[width=9cm]{points/kmalek_179.eps}
\includegraphics[width=9cm]{points/kmalek_181.eps}
\includegraphics[width=9cm]{points/kmalek_183.eps}
\includegraphics[width=9cm]{points/kmalek_184.eps}
\includegraphics[width=9cm]{points/kmalek_185.eps}
\includegraphics[width=9cm]{points/kmalek_190.eps}
\includegraphics[width=9cm]{points/kmalek_191.eps}
\includegraphics[width=9cm]{points/kmalek_192.eps}
\includegraphics[width=9cm]{points/kmalek_194.eps}
\includegraphics[width=9cm]{points/kmalek_195.eps}
\includegraphics[width=9cm]{points/kmalek_196.eps}
\includegraphics[width=9cm]{points/kmalek_198.eps}
\includegraphics[width=9cm]{points/kmalek_199.eps}
\includegraphics[width=9cm]{points/kmalek_200.eps}
\includegraphics[width=9cm]{points/kmalek_201.eps}
\includegraphics[width=9cm]{points/kmalek_203.eps}
\includegraphics[width=9cm]{points/kmalek_204.eps}
\includegraphics[width=9cm]{points/kmalek_205.eps}
\includegraphics[width=9cm]{points/kmalek_206.eps}
\includegraphics[width=9cm]{points/kmalek_210.eps}
\includegraphics[width=9cm]{points/kmalek_211.eps}
\includegraphics[width=9cm]{points/kmalek_212.eps}
\includegraphics[width=9cm]{points/kmalek_213.eps}
\includegraphics[width=9cm]{points/kmalek_214.eps}
\includegraphics[width=9cm]{points/kmalek_215.eps}
\includegraphics[width=9cm]{points/kmalek_216.eps}
\includegraphics[width=9cm]{points/kmalek_218.eps}
\includegraphics[width=9cm]{points/kmalek_219.eps}
\includegraphics[width=9cm]{points/kmalek_222.eps}
\includegraphics[width=9cm]{points/kmalek_223.eps}
\includegraphics[width=9cm]{points/kmalek_224.eps}
\includegraphics[width=9cm]{points/kmalek_225.eps}
\includegraphics[width=9cm]{points/kmalek_226.eps}
\includegraphics[width=9cm]{points/kmalek_228.eps}
\includegraphics[width=9cm]{points/kmalek_232.eps}
\includegraphics[width=9cm]{points/kmalek_233.eps}
\includegraphics[width=9cm]{points/kmalek_234.eps}
\includegraphics[width=9cm]{points/kmalek_239.eps}
\includegraphics[width=9cm]{points/kmalek_244.eps}
\includegraphics[width=9cm]{points/kmalek_247.eps}
\includegraphics[width=9cm]{points/kmalek_252.eps}
\includegraphics[width=9cm]{points/kmalek_253.eps}
\includegraphics[width=9cm]{points/kmalek_254.eps}
\includegraphics[width=9cm]{points/kmalek_255.eps}
\includegraphics[width=9cm]{points/kmalek_256.eps}
\includegraphics[width=9cm]{points/kmalek_257.eps}
\includegraphics[width=9cm]{points/kmalek_258.eps}
\includegraphics[width=9cm]{points/kmalek_259.eps}
\includegraphics[width=9cm]{points/kmalek_260.eps}
\includegraphics[width=9cm]{points/kmalek_261.eps}
\includegraphics[width=9cm]{points/kmalek_262.eps}
\includegraphics[width=9cm]{points/kmalek_265.eps}
\includegraphics[width=9cm]{points/kmalek_267.eps}
\includegraphics[width=9cm]{points/kmalek_270.eps}
\includegraphics[width=9cm]{points/kmalek_271.eps}
\includegraphics[width=9cm]{points/kmalek_275.eps}
\includegraphics[width=9cm]{points/kmalek_277.eps}
\includegraphics[width=9cm]{points/kmalek_279.eps}
\includegraphics[width=9cm]{points/kmalek_280.eps}
\includegraphics[width=9cm]{points/kmalek_281.eps}
\includegraphics[width=9cm]{points/kmalek_283.eps}
\includegraphics[width=9cm]{points/kmalek_287.eps}
\includegraphics[width=9cm]{points/kmalek_288.eps}
\includegraphics[width=9cm]{points/kmalek_290.eps}
\includegraphics[width=9cm]{points/kmalek_292.eps}
\includegraphics[width=9cm]{points/kmalek_294.eps}
\includegraphics[width=9cm]{points/kmalek_295.eps}
\includegraphics[width=9cm]{points/kmalek_297.eps}
\includegraphics[width=9cm]{points/kmalek_299.eps}
\includegraphics[width=9cm]{points/kmalek_300.eps}
\includegraphics[width=9cm]{points/kmalek_301.eps}
\includegraphics[width=9cm]{points/kmalek_302.eps}
\includegraphics[width=9cm]{points/kmalek_304.eps}
\includegraphics[width=9cm]{points/kmalek_306.eps}
\includegraphics[width=9cm]{points/kmalek_307.eps}
\includegraphics[width=9cm]{points/kmalek_308.eps}
\includegraphics[width=9cm]{points/kmalek_310.eps}
\includegraphics[width=9cm]{points/kmalek_311.eps}
\includegraphics[width=9cm]{points/kmalek_312.eps}
\includegraphics[width=9cm]{points/kmalek_314.eps}
\includegraphics[width=9cm]{points/kmalek_317.eps}
\includegraphics[width=9cm]{points/kmalek_318.eps}
\includegraphics[width=9cm]{points/kmalek_323.eps}
\includegraphics[width=9cm]{points/kmalek_324.eps}
\includegraphics[width=9cm]{points/kmalek_327.eps}
\includegraphics[width=9cm]{points/kmalek_328.eps}
\includegraphics[width=9cm]{points/kmalek_329.eps}
\includegraphics[width=9cm]{points/kmalek_334.eps}
\includegraphics[width=9cm]{points/kmalek_335.eps}
\includegraphics[width=9cm]{points/kmalek_336.eps}
\includegraphics[width=9cm]{points/kmalek_337.eps}
\includegraphics[width=9cm]{points/kmalek_338.eps}
\includegraphics[width=9cm]{points/kmalek_339.eps}
\includegraphics[width=9cm]{points/kmalek_340.eps}
\includegraphics[width=9cm]{points/kmalek_341.eps}
\includegraphics[width=9cm]{points/kmalek_342.eps}
\includegraphics[width=9cm]{points/kmalek_343.eps}
\includegraphics[width=9cm]{points/kmalek_344.eps}
\includegraphics[width=9cm]{points/kmalek_345.eps}
\includegraphics[width=9cm]{points/kmalek_348.eps}
\includegraphics[width=9cm]{points/kmalek_351.eps}
\includegraphics[width=9cm]{points/kmalek_352.eps}
\includegraphics[width=9cm]{points/kmalek_354.eps}
\includegraphics[width=9cm]{points/kmalek_355.eps}
\includegraphics[width=9cm]{points/kmalek_357.eps}
\includegraphics[width=9cm]{points/kmalek_358.eps}
\includegraphics[width=9cm]{points/kmalek_360.eps}
\includegraphics[width=9cm]{points/kmalek_364.eps}
\includegraphics[width=9cm]{points/kmalek_365.eps}
\includegraphics[width=9cm]{points/kmalek_366.eps}
\includegraphics[width=9cm]{points/kmalek_368.eps}
\includegraphics[width=9cm]{points/kmalek_369.eps}
\includegraphics[width=9cm]{points/kmalek_370.eps}
\includegraphics[width=9cm]{points/kmalek_373.eps}
\includegraphics[width=9cm]{points/kmalek_374.eps}
\includegraphics[width=9cm]{points/kmalek_377.eps}
\includegraphics[width=9cm]{points/kmalek_380.eps}
\includegraphics[width=9cm]{points/kmalek_384.eps}
\includegraphics[width=9cm]{points/kmalek_386.eps}
\includegraphics[width=9cm]{points/kmalek_391.eps}
\includegraphics[width=9cm]{points/kmalek_392.eps}
\includegraphics[width=9cm]{points/kmalek_393.eps}
\includegraphics[width=9cm]{points/kmalek_394.eps}
\includegraphics[width=9cm]{points/kmalek_396.eps}
\includegraphics[width=9cm]{points/kmalek_397.eps}
\includegraphics[width=9cm]{points/kmalek_398.eps}
\includegraphics[width=9cm]{points/kmalek_399.eps}
\includegraphics[width=9cm]{points/kmalek_400.eps}
\includegraphics[width=9cm]{points/kmalek_402.eps}
\includegraphics[width=9cm]{points/kmalek_410.eps}
\includegraphics[width=9cm]{points/kmalek_414.eps}
\includegraphics[width=9cm]{points/kmalek_415.eps}
\includegraphics[width=9cm]{points/kmalek_416.eps}
\includegraphics[width=9cm]{points/kmalek_418.eps}
\includegraphics[width=9cm]{points/kmalek_419.eps}
\includegraphics[width=9cm]{points/kmalek_422.eps}
\includegraphics[width=9cm]{points/kmalek_423.eps}
\includegraphics[width=9cm]{points/kmalek_424.eps}
\includegraphics[width=9cm]{points/kmalek_426.eps}
\includegraphics[width=9cm]{points/kmalek_430.eps}
\includegraphics[width=9cm]{points/kmalek_431.eps}
\includegraphics[width=9cm]{points/kmalek_432.eps}
\includegraphics[width=9cm]{points/kmalek_434.eps}
\includegraphics[width=9cm]{points/kmalek_436.eps}
\includegraphics[width=9cm]{points/kmalek_437.eps}
\includegraphics[width=9cm]{points/kmalek_439.eps}
\includegraphics[width=9cm]{points/kmalek_441.eps}
\includegraphics[width=9cm]{points/kmalek_443.eps}
\includegraphics[width=9cm]{points/kmalek_445.eps}
\includegraphics[width=9cm]{points/kmalek_447.eps}
\includegraphics[width=9cm]{points/kmalek_448.eps}
\includegraphics[width=9cm]{points/kmalek_449.eps}
\includegraphics[width=9cm]{points/kmalek_450.eps}
\includegraphics[width=9cm]{points/kmalek_451.eps}
\includegraphics[width=9cm]{points/kmalek_452.eps}
\includegraphics[width=9cm]{points/kmalek_458.eps}
\includegraphics[width=9cm]{points/kmalek_460.eps}
\includegraphics[width=9cm]{points/kmalek_462.eps}
\includegraphics[width=9cm]{points/kmalek_463.eps}
\includegraphics[width=9cm]{points/kmalek_464.eps}
\includegraphics[width=9cm]{points/kmalek_465.eps}
\includegraphics[width=9cm]{points/kmalek_466.eps}
\includegraphics[width=9cm]{points/kmalek_467.eps}
\includegraphics[width=9cm]{points/kmalek_468.eps}
\includegraphics[width=9cm]{points/kmalek_472.eps}
\includegraphics[width=9cm]{points/kmalek_473.eps}
\includegraphics[width=9cm]{points/kmalek_474.eps}
\includegraphics[width=9cm]{points/kmalek_477.eps}
\includegraphics[width=9cm]{points/kmalek_482.eps}
\includegraphics[width=9cm]{points/kmalek_486.eps}
\includegraphics[width=9cm]{points/kmalek_488.eps}
\includegraphics[width=9cm]{points/kmalek_489.eps}
\includegraphics[width=9cm]{points/kmalek_490.eps}
\includegraphics[width=9cm]{points/kmalek_492.eps}
\includegraphics[width=9cm]{points/kmalek_493.eps}
\includegraphics[width=9cm]{points/kmalek_494.eps}
\includegraphics[width=9cm]{points/kmalek_496.eps}
\includegraphics[width=9cm]{points/kmalek_497.eps}
\includegraphics[width=9cm]{points/kmalek_499.eps}
\includegraphics[width=9cm]{points/}

